RISs and Sidelink Communications in Smart Cities: The Key to Seamless Localization and Sensing

A smart city involves, among other elements, intelligent transportation, crowd monitoring, and digital twins, each of which requires information exchange via wireless communication links and localization of connected devices and passive objects (including people). Although localization and sensing (L&S) are envisioned as core functions of future communication systems, they have inherently different demands in terms of infrastructure compared to communications. Wireless communications generally requires a connection to only a single access point (AP), while L&S demand simultaneous line-of-sight propagation paths to several APs, which serve as location and orientation anchors. Hence, a smart city deployment optimized for communication will be insufficient to meet stringent L&S requirements. In this article, we argue that the emerging technologies of reconfigurable intelligent surfaces (RISs) and sidelink communications constitute the key to providing ubiquitous coverage for L&S in smart cities with low-cost and energy-efficient technical solutions. To this end, we propose and evaluate AP-coordinated and self-coordinated RIS-enabled L&S architectures and detail three groups of application scenarios, relying on low-complexity beacons, cooperative localization, and full-duplex transceivers. A list of practical issues and consequent open research challenges of the proposed L&S systems is also provided.

==> Figures/PEBvsUncert.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
\definecolor{mycolor1}{rgb}{0.46667,0.67451,0.18824}%
%
\begin{tikzpicture}

\begin{axis}[%
% width=76mm,
% height=40mm,
width=75mm,
height=30mm,
% height=25mm,
at={(0mm,0mm)},
scale only axis,
xmin=0,
xmax=10,
% xlabel style={font=\color{white!15!black}},
% xlabel={UE uncertainty [m]},
ymin=0.1,
ymax=100,
ymode=log,
yticklabel style = {font=\small,xshift=0.5ex},
xticklabel style = {font=\small,yshift=0ex},
% ylabel style={font=\color{white!15!black}},
% ylabel={Position Est. (MAE) [m]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend pos=south east,legend cell align=left, align=left, draw=white!15!black,style={row sep=-0.1cm}}
]

\addplot [color=mycolor1, line width=1.0pt, mark=+, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0.01	8.65877159329929\\
0.1	8.65877159329929\\
0.2	8.65877159329929\\
0.3	8.65877159329929\\
0.4	8.65877159329929\\
0.5	8.65877159329929\\
0.6	8.65877159329929\\
0.7	8.65877159329929\\
0.8	8.65877159329929\\
0.9	8.65877159329929\\
1	8.65877159329929\\
2	8.65877159329929\\
3	8.65877159329929\\
4	8.65877159329929\\
5	8.65877159329929\\
6	8.65877159329929\\
7	8.65877159329929\\
8	8.65877159329929\\
9	8.65877159329929\\
10	8.65877159329929\\
};
\addlegendentry{\footnotesize{Random profile}}

\addplot [color=blue, line width=1.0pt, mark=o, mark options={solid, blue}]
  table[row sep=crcr]{%
0.01	38.1291485915582\\
0.1	3.83817300437474\\
0.2	1.95623600895186\\
0.3	1.34602295007486\\
0.4	1.05487735647951\\
0.5	0.892688458674215\\
0.6	0.796468179805877\\
0.7	0.739569093660476\\
0.8	0.708958941989795\\
0.9	0.697587462226162\\
1	0.70123022078779\\
2	0.933885725560279\\
3	1.40506403501427\\
4	2.57523978493561\\
5	3.41729525539841\\
6	4.5226780275594\\
7	7.55794201972935\\
8	9.35799551929238\\
9	12.9557113685996\\
10	15.3668815728465\\
};
\addlegendentry{\footnotesize Directional profile}

% \addplot [color=red, dashed, line width=1.0pt, mark=x, mark options={solid, red}]
%   table[row sep=crcr]{%
% 0.01	20.5525006524443\\
% 0.1	2.07428346391296\\
% 0.2	1.06005427858459\\
% 0.3	0.731045941539933\\
% 0.4	0.57377833331909\\
% 0.5	0.485603862492259\\
% 0.6	0.432307643032828\\
% 0.7	0.399204731442262\\
% 0.8	0.378952818858566\\
% 0.9	0.367520085013714\\
% 1	0.362576804618955\\
% 2	0.517474278738619\\
% 3	0.884428595977512\\
% 4	1.39128913922309\\
% 5	1.98592806433056\\
% 6	2.58726733523046\\
% 7	2.96151556131542\\
% 8	3.33970062513529\\
% 9	3.74158112155263\\
% 10	5.74652283463067\\
% };
% \addlegendentry{\footnotesize Uniform profile (proposed)}

\end{axis}

% \node[rotate=0,fill=white] (BOC6) at (3.9cm,-.65cm){\small UE uncertainty [m]};
% \node[rotate=90] at (-8mm,2cm){\small PEB [m]};
\node[rotate=0,fill=white] (BOC6) at (3.35cm,-.7cm){\small UE uncertainty [m]};
\node[rotate=90] at (-8mm,12.5mm){\small PEB [m]};
% \node[rotate=90] at (-8mm,2cm){\small PEB [m]};

\end{tikzpicture}%

==> acronyms_full.tex <==
% \newlist{acronyms}{description}{1}
% \setlist[acronyms]{
% labelwidth = 4.5em,
% leftmargin = 5em,
% noitemsep,
% itemindent = 0pt}
% \DeclareAcroListStyle{mystyle}{list}{ list = acronyms }
% \acsetup{ list-style = mystyle }

\DeclareAcronym{5g}{
short=5G,
long= fifth generation,
}
\DeclareAcronym{6g}{
short=6G,
long= sixth generation,
}
\DeclareAcronym{3d}{
short=3D,
long= three-dimensional,
}
\DeclareAcronym{ace}{
short=ACE,
long= array calibration error,
}
\DeclareAcronym{alb}{
short=ALB,
long= absolute lower bound,
}
\DeclareAcronym{aod}{
short=AOD,
long= angle-of-departure,
}
\DeclareAcronym{aosa}{
short=AOSA,
long= array-of-subarray,
}
\DeclareAcronym{adod}{
short=ADOD,
long= angle-difference-of-departure,
}
\DeclareAcronym{aoa}{
short=AOA,
long= angle-of-arrival,
}
\DeclareAcronym{adc}{
short=ADC,
long= analog to digital converter,
}
\DeclareAcronym{aeb}{
short=AEB,
long= angle error bound,
}
\DeclareAcronym{age}{
short=AGE,
long= array gain error,
}
\DeclareAcronym{ade}{
short=ADE,
long= antenna displacement error,
}
\DeclareAcronym{av}{
short=AV,
long= autonomous vehicle,
}
\DeclareAcronym{ap}{
short=AP,
long= access point,
}
\DeclareAcronym{bs}{
short=BS,
long= base station,
}
\DeclareAcronym{bse}{
short=BSE,
long= beam split effect,
}
\DeclareAcronym{csi}{
short=CSI,
long= channel state information,
}
\DeclareAcronym{cfo}{
short=CFO,
long= carrier frequency offset,
}
\DeclareAcronym{ceb}{
short=CEB,
long= clock error bound,
}
\DeclareAcronym{coa}{
short=COA,
long= curvature-of-arrival,
}
\DeclareAcronym{crb}{
short=CRB,
long= Cram\'er-Rao bound,
}
\DeclareAcronym{ccrb}{
short=CCRB,
long= constrained Cram\'er-Rao bound,
}
\DeclareAcronym{cmos}{
short=CMOS,
long= complementary metal-oxide-semiconductor,
}
\DeclareAcronym{crlb}{
short=CRLB,
long= Cram\'er-Rao lower bound,
}
\DeclareAcronym{cdf}{
short=CDF,
long= cumulative distribution function,
}
\DeclareAcronym{cp}{
short=CP,
long= cyclic prefix,
}
\DeclareAcronym{dac}{
short=DAC,
long= digital to analog converter,
}
\DeclareAcronym{dfl}{
short=DFL,
long= device-free localization,
}
\DeclareAcronym{dmimo}{
short=D-MIMO,
long= distributed MIMO,
}
\DeclareAcronym{dlprs}{
short=DL-PRS,
long= downlink positioning reference signal,
}
\DeclareAcronym{d2d}{
short=D2D,
long= device-to-device,
}
\DeclareAcronym{dftsofdm}{
short=DFT-s-OFDM,
long= discrete-Fourier-transform spread OFDM,
}
\DeclareAcronym{dl}{
short=DL,
long= deep learning,
}
\DeclareAcronym{gps}{
short=GPS,
long= global positioning system,
}
\DeclareAcronym{gnss}{
short=GNSS,
long= global navigation satellite system,
}
\DeclareAcronym{hwi}{
short=HWI,
long= hardware impairment,
}
\DeclareAcronym{hemt}{
short=HEMT,
long= high electron mobility transistor,
}
\DeclareAcronym{hbt}{
short=HBT,
long= heterojunction bipolar transistors,
}
\DeclareAcronym{iot}{
short=IoT,
long= internet of things,
}
\DeclareAcronym{isac}{
short=ISAC,
long= integrated sensing and communication,
}
\DeclareAcronym{iqi}{
short=IQI,
long= in-phase and quadrature imbalance,
}
\DeclareAcronym{ia}{
short=IA,
long= initial access,
}
\DeclareAcronym{kpi}{
short=KPI,
long= key performance indicator,
}
\DeclareAcronym{kf}{
short=KF,
long= Kalman filter,
}
\DeclareAcronym{ekf}{
short=EKF,
long= extended Kalman filter,
}
\DeclareAcronym{ukf}{
short=UKF,
long= unscented Kalman filter,
}
\DeclareAcronym{ckf}{
short=CKF,
long= cubature Kalman filter,
}
\DeclareAcronym{pf}{
short=PF,
long= particle filter,
}
\DeclareAcronym{lb}{
short=LB,
long= lower bound,
}
\DeclareAcronym{lse}{
short=LSE,
long= least-square estimator,
}
\DeclareAcronym{lo}{
short=LO,
long= local oscillator,
}
\DeclareAcronym{los}{
short=LOS,
long= line-of-sight,
}
\DeclareAcronym{mc}{
short=MC,
long= mutual coupling,
}
\DeclareAcronym{mac}{
short=MAC,
long= medium access control,
}
\DeclareAcronym{meb}{
short=MEB,
long= mapping error bound,
}
\DeclareAcronym{ml}{
short=ML,
long= machine learning,
}
\DeclareAcronym{mcrb}{
short=MCRB,
long= misspecified Cram\'er-Rao bound,
}
\DeclareAcronym{mds}{
short=MDS,
long= multidimensional scaling ,
}
\DeclareAcronym{mimo}{
short=MIMO,
long= multiple-input-multiple-output,
}
\DeclareAcronym{mm}{
short=MM,
long= mismatched model,
}
\DeclareAcronym{mpc}{
short=MPC,
long= multipath component,
}
\DeclareAcronym{mmwave}{
short=mmWave,
long= millimeter wave,
}
\DeclareAcronym{mmle}{
short=MMLE,
long= mismatched maximum likelihood estimation,
}
\DeclareAcronym{mems}{
short=MEMS,
long= micro-electro-mechanical system,
}
\DeclareAcronym{mle}{
short=MLE,
long= maximum likelihood estimation,
}
\DeclareAcronym{nlos}{
short=NLOS,
long= none-line-of-sight,
}
\DeclareAcronym{ofdm}{
short=OFDM,
long= orthogonal frequency-division multiplexing,
}
\DeclareAcronym{oeb}{
short=OEB,
long= orientation error bound,
}
\DeclareAcronym{otfs}{
short=OTFS,
long= orthogonal time-frequency space,
}
\DeclareAcronym{pdf}{
short=PDF,
long= probability density function,
}
\DeclareAcronym{papr}{
short=PAPR,
long= peak-to-average-power ratio,
}
\DeclareAcronym{pan}{
short=PAN,
long= power amplifier nonlinearity,
}
\DeclareAcronym{pa}{
short=PA,
long= power amplifier,
}
\DeclareAcronym{ps}{
short=PS,
long= phase shifter,
}
\DeclareAcronym{pn}{
short=PN,
long= phase noise,
}
\DeclareAcronym{poa}{
short=POA,
long= phase-of-arrival,
}
\DeclareAcronym{pwm}{
short=PWM,
long= planar wave model,
}
\DeclareAcronym{pdoa}{
short=PDOA,
long= phase-difference-of-arrival,
}
\DeclareAcronym{prs}{
short=PRS,
long= positioning reference signals,
}
\DeclareAcronym{peb}{
short=PEB,
long= position error bound,
}
\DeclareAcronym{qam}{
short=QAM,
long= quadrature amplitude modulation,
}
\DeclareAcronym{rnn}{
short=RNN,
long= recurrent neural network,
}
\DeclareAcronym{rl}{
short=RL,
long= reinforcement learning,
}
\DeclareAcronym{rfc}{
short=RFC,
long= radio-frequency chain,
}
\DeclareAcronym{rf}{
short=RF,
long= radio frequency,
}
\DeclareAcronym{rfid}{
short=RFID,
long= radio frequency identification,
}
\DeclareAcronym{ris}{
short=RIS,
long= reconfigurable intelligent surface,
}
\DeclareAcronym{rss}{
short=RSS,
long= received signal strength,
}
\DeclareAcronym{rtt}{
short=RTT,
long= round-trip time,
}
\DeclareAcronym{sm}{
short=SM,
long= standard model,
}
\DeclareAcronym{sige}{
short=SiGe,
long= silicon-germanium,
}
\DeclareAcronym{spp}{
short=SPP,
long= surface plasmon polariton,
}
\DeclareAcronym{sa}{
short=SA,
long= subarray,
}
\DeclareAcronym{ser}{
short=SER,
long= symbol error rate,
}
\DeclareAcronym{simo}{
short=SIMO,
long= single-input-multiple-output,
}
\DeclareAcronym{sota}{
short=SOTA,
long= state-of-the-art,
}
\DeclareAcronym{swm}{
short=SWM,
long= spherical wave model,
}
\DeclareAcronym{slam}{
short=SLAM,
long= simultaneous localization and mapping,
}
\DeclareAcronym{tm}{
short=TM,
long= true model,
}
\DeclareAcronym{toa}{
short=TOA,
long= time-of-arrival,
}
\DeclareAcronym{tof}{
short=TOF,
long= time-of-flight,
}
\DeclareAcronym{tdoa}{
short=TDOA,
long= time-difference-of-arrival,
}
\DeclareAcronym{thz}{
short=THz,
long= terahertz,
}
\DeclareAcronym{ue}{
short=UE,
long= user equipment,
}
\DeclareAcronym{ummimo}{
short=UM-MIMO,
long= ultra-massive multi-input-multi-output,
}
\DeclareAcronym{vlp}{
short=VLP,
long= visible light positioning,
}
\DeclareAcronym{veb}{
short=VEB,
long= velocity error bound,
}
\DeclareAcronym{vlc}{
short=VLC,
long= visible light communication,
}
\DeclareAcronym{ula}{
short=ULA,
long= uniform linear array,
}
\DeclareAcronym{upa}{
short=UPA,
long= uniform planar array,
}
\DeclareAcronym{wlan}{
short=WLAN,
long= wireless local area network,
}





% Abbreviations for Conferences
% @STRING{ICASSP         = "Proc. IEEE Int. Conf. Acoustics, Speech, and Signal Process. (ICASSP)"}
% @STRING{VTC            = "Proc. IEEE Vehic. Technol. Conf. (VTC)"}
% @STRING{ICC            = "Proc. IEEE Int. Conf. Commun. (ICC)"}
% @STRING{ISCAS          = "Proc. IEEE Int. Symp. on Circuits and Systems (ISCAS)"}
% @STRING{WCNC           = "Proc. IEEE Wireless Commun. and Netw. Conf. (WCNC)"}
% @STRING{ASILOMAR       = "Proc. Asilomar Conf. Signals, Systems and Computers (Asilomar)"}
% @STRING{PIMRC          = "Proc. IEEE Int. Symp. Personal Indoor and Mobile Radio Commun. (PIMRC)"}
% @string{GLOBECOM       = "Proc. IEEE Global Conmun. Conf. (GLOBECOM)"}
% @string{MILCOM         = "Proc. IEEE MILCOM"}
% @string{GlobalSIP      = "Proc. IEEE Global Conf. on Signal and Inform. Process. (GlobalSIP)"}
% @string{SPIE      = "Proc. SPIE"}

% IEEE Journals

% aerospace and military
% @STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
% @STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
% @STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
% @STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
% @STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
% @STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



% autos, transportation and vehicles (non-aerospace)
% @STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transp. Syst."}
% @STRING{IEEE_J_IV         = "{IEEE} Trans. Intell. Veh."}
% @STRING{IEEE_J_TTE        = "{IEEE} Trans. Transport. Electrific."}
% @STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}
% @STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}



% circuits, signals, systems, audio and controls
% @STRING{IEEE_J_STSP       = "{IEEE} J. Sel. Topics Signal Process."}
% @STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}
% @STRING{IEEE_J_SYST       = "{IEEE} Syst. J."}
% @STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}
% @STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
% @STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
% in 2014 ASL became ASLP
% @STRING{IEEE_J_ASLP       = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
% @STRING{IEEE_J_ASL        = "{IEEE} Audio, Speech, Language Process."}
% @STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Control"}
% @STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
% @STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
% @STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
% @STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
% @STRING{IEEE_J_CASI_RP    = "{IEEE} Trans. Circuits Syst. {I}"}
% @STRING{IEEE_J_CASII_EB   = "{IEEE} Trans. Circuits Syst. {II}"}
% @STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
% @STRING{IEEE_J_CST        = "{IEEE} Trans. Control Syst. Technol."}
% @STRING{IEEE_J_ETCAS      = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
% @STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}
% @STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
% @STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}
% @STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
% @STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}



% communications
% @STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
% @STRING{IEEE_J_JSAC       = "{IEEE} J. Sel. Areas Commun."}
% @STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
% @STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
% @STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}
% @STRING{IEEE_J_WCOML      = "{IEEE} Wireless Commun. Lett."}


% coding, data, information, knowledge
% @STRING{IEEE_J_BD         = "{IEEE} Trans. Big Data"}
% @STRING{IEEE_J_IFS        = "{IEEE} Trans. Inf. Forensics Security"}
% @STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}
% @STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}


% computers, computation, networking and software
% @STRING{IEEE_J_CAL        = "{IEEE} Comput. Archit. Lett."}
% @STRING{IEEE_J_ES         = "{IEEE} Embedded Syst. Lett."}
% @STRING{IEEE_J_IOT        = "{IEEE} Internet Things J."}
% @STRING{IEEE_J_XCDC       = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
% @STRING{IEEE_J_MMCT       = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
% @STRING{IEEE_J_SUSC       = "{IEEE} Sustain. Comput."}
% @STRING{IEEE_J_CC         = "{IEEE} Trans. on Cloud Comput."}
% @STRING{IEEE_J_CSS        = "{IEEE} Trans. Comput. Social Syst."}
% @STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
% @STRING{IEEE_J_CNS        = "{IEEE} Trans. Control Netw. Syst."}
% @STRING{IEEE_J_DSC        = "{IEEE} Trans. Depend. Sec. Comput."}
% @STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
% @STRING{IEEE_J_ETC        = "{IEEE} Trans. Emerg. Topics Comput."}
% @STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
% @STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
% @STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
% @STRING{IEEE_J_MSCS       = "{IEEE} Trans. Multi-Scale Comput. Syst."}
% @STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Netw."}
% @STRING{IEEE_J_NSE        = "{IEEE} Trans. Netw. Sci. Eng."}
% @STRING{IEEE_J_NSM        = "{IEEE} Trans. Netw. Service Manag."}
% @STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
% in 2012 NN became NNLS
% @STRING{IEEE_J_NNLS       = "{IEEE} Trans. Neural Netw. Learn. Syst."}
% @STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
% @STRING{IEEE_J_SC         = "{IEEE} Trans. Serv. Comput."}
% @STRING{IEEE_J_SIPN       = "{IEEE} Trans. Signal Inf. Process. Netw."}
% @STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}


% computer graphics, imaging, and multimedia
% @STRING{IEEE_J_JDT        = "{IEEE/OSA} J. Display Technol."}
% @STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}
% @STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
% @STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}


% cybernetics, ergonomics, robots, man-machine, artificial intelligence and automation
% @STRING{IEEE_J_JAS        = "{IEEE/CAA} J. Autom. Sinica"}
% @STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
% @STRING{IEEE_J_AFFC       = "{IEEE} Trans. Affect. Comput."}
% @STRING{IEEE_J_ASE        = "{IEEE} Trans. Autom. Sci. Eng."}
% @STRING{IEEE_J_AMD        = "{IEEE} Trans. Auton. Mental Develop."}
% @STRING{IEEE_J_CCN        = "{IEEE} Trans. on Cogn. Commun. Netw."}
% in 2015 AMD became CDS
% @STRING{IEEE_J_CDS        = "{IEEE} Trans. Cogn. Develop. Syst."}
% @STRING{IEEE_J_CIAIG      = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
% in 2013 SMCB became CYB
% @STRING{IEEE_J_CYB        = "{IEEE} Trans. Cybern."}
% @STRING{IEEE_J_H          = "{IEEE} Trans. Haptics"}
% @STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
% in 2013 SMCC became HMS
% @STRING{IEEE_J_HMS        = "{IEEE} Trans. Human-Mach. Syst."}
% @STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
% @STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
% in 1989 JRA became RA
% in August 2004, RA split into ASE and RO
% @STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}
% @STRING{IEEE_J_RAL        = "{IEEE} Robot. Autom. Lett."}
% @STRING{IEEE_J_RO         = "{IEEE} Trans. Robot."}
% @STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
% @STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
% @STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
% @STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
% in 2012 SMCA became SMCS
% @STRING{IEEE_J_SMCS       = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
% @STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}


% education, engineering, history, IEEE, professional
% @STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
% @STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
% @STRING{IEEE_J_RITA       = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
% @STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
% @STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manag."}
% @STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
% @STRING{IEEE_J_LT         = "{IEEE} Trans. Learn. Technol."}
% @STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}

% electromagnetics, antennas, EMI, magnetics and microwave
% @STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propag. Lett."}
% @STRING{IEEE_J_MAGL       = "{IEEE} Magn. Lett."}
% @STRING{IEEE_J_MGWL       = "{IEEE} Microw. Guided Wave Lett."}
% @STRING{IEEE_J_MWCL       = "{IEEE} Microw. Wireless Compon. Lett."}
% @STRING{IEEE_J_RFIC       = "{IEEE} {RFIC} J."}
% @STRING{IEEE_J_RFID       = "{IEEE} {RFID} J."}
% @STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propag."}
% @STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
% @STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
% @STRING{IEEE_J_MTT        = "{IEEE} Trans. Microw. Theory Techn."}
% @STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
% @STRING{IEEE_J_TTHZ       = "{IEEE} Trans. {THz} Sci. Technol."}
% @STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}


% industrial, commercial and consumer
% @STRING{IEEE_J_PSE        = "{IEEE} J. Product Safety Eng."}
% @STRING{IEEE_J_APPIND     = "{IEEE} Trans. Appl. Ind."}
% @STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
% @STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
% @STRING{IEEE_J_CE         = "{IEEE} Trans. Consum. Electron."}
% @STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
% @STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
% @STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Appl."}
% @STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Appl."}
% @STRING{IEEE_J_IINF       = "{IEEE} Trans. Ind. Informat."}

% instrumentation and measurement
% @STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}


% optics, lightwave and photonics
% @STRING{IEEE_J_JLT        = "J. Lightw. Technol."}
% @STRING{IEEE_J_OCN        = "{IEEE} J. Opt. Commun. Netw."}
% @STRING{IEEE_J_PJ         = "{IEEE} Photon. J."}
% @STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}


% sensors
% @STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}


% IEEE Magazines and Online Publications


% @STRING{IEEE_O_ACC        = "{IEEE} Access"}
% @STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag."}
% @STRING{IEEE_M_HIST       = "{IEEE} Ann. Hist. Comput."}
% @STRING{IEEE_M_AP         = "{IEEE} Antennas Propag. Mag."}
% @STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
% @STRING{IEEE_M_CHINAC     = "China Commun."}
% @STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
% @STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
% @STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
% @STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
% @STRING{IEEE_O_CSTO       = "{IEEE} Commun. Surveys Tuts."}
% @STRING{IEEE_M_CIM        = "{IEEE} Comput. Intell. Mag."}
% CSEM changed to CSE in 1999
% @STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
% @STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
% @STRING{IEEE_M_C          = "Computer"}
% @STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
% @STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
% @STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
% @STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
% in 2012 DTC became DT
% @STRING{IEEE_M_DT         = "{IEEE} Des. Test"}
% @STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
% @STRING{IEEE_O_DSO        = "{IEEE} Distrib. Syst. Online"}
% @STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
% @STRING{IEEE_M_ETF        = "{IEEE} Electrific. Mag."}
% @STRING{IEEE_M_EMC        = "{IEEE} Electromagn. Compat."}
% @STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnol. Rev."}
% @STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
% @STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
% @STRING{IEEE_M_EXP        = "{IEEE} Expert"}
% @STRING{IEEE_M_GRS        = "{IEEE} Geosci. Remote Sens. Mag."}
% @STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
% @STRING{IEEE_M_IE         = "{IEEE} Ind. Electron. Mag."}
% @STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
% @STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
% @STRING{IEEE_M_ITS        = "{IEEE} Intell. Transp. Syst. Mag."}
% @STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
% @STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
% @STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
% @STRING{IEEE_M_MW         = "{IEEE} Microw. Mag."}
% @STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
% @STRING{IEEE_M_NANO       = "{IEEE} Nanotechnol. Mag."}
% @STRING{IEEE_M_NET        = "{IEEE} Netw."}
% IEEE's editorial manual lists "Pers. Commun.",
% but "Personal Commun. Mag." seems to be what is used in the journals
% @STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
% @STRING{IEEE_M_PVC        = "{IEEE} Pervasive Comput."}
% @STRING{IEEE_M_POT        = "{IEEE} Potentials"}
% @STRING{IEEE_M_PEL        = "{IEEE} Power Electron. Mag."}
% CAP and PER merged to form PE in 2003
% @STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
% @STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
% @STRING{IEEE_M_PULSE      = "{IEEE} Pulse"}
% @STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
% @STRING{IEEE_M_SAP        = "{IEEE} Security Privacy"}
% @STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
% @STRING{IEEE_M_S          = "{IEEE} Softw."}
% @STRING{IEEE_M_SSC        = "{IEEE} Solid-State Circuits Mag."}
% @STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
% @STRING{IEEE_M_SMC        = "{IEEE} Syst., Man, Cybern. Mag."}
% @STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
% @STRING{IEEE_M_VT         = "{IEEE} Veh. Technol. Mag."}
% @STRING{IEEE_M_WC         = "{IEEE} Wireless Commun."}






















==> macros.tex <==

%
\setlength\unitlength{1mm}

\newcommand{\insertfig}[3]{
\begin{figure}[htbp]\begin{center}\begin{picture}(120,90)
\put(0,-5){\includegraphics[width=12cm,height=9cm,clip=]{#1.eps}}\end{picture}\end{center}
\caption{#2}\label{#3}\end{figure}}

\newcommand{\insertxfig}[4]{
\begin{figure}[htbp]
\begin{center}
\leavevmode \centerline{\resizebox{#4\textwidth}{!}{\input
#1.pstex_t}}
%\vspace*{-0.2in}
\caption{#2} \label{#3}
\end{center}
\end{figure}}

\long\def\comment#1{}


% bb font symbols
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newfont{\bbb}{msbm10 scaled 700}
\newcommand{\CCC}{\mbox{\bbb C}}
\newcommand{\ssn}[1]{{\scriptscriptstyle{{#1}}}}
\newcommand{\ssr}[1]{{\scriptscriptstyle{\mathrm{#1}}}}
\newcommand{\ssnb}[1]{{\scriptscriptstyle{({#1})}}}
\newcommand{\ssrb}[1]{{\scriptscriptstyle{(\mathrm{#1})}}}

% replace `c' with `!\vthickline'
% replace \hline with \hthickline
\newcommand{\vthickline}{\vrule width 0.8pt}
\newcommand{\hthickline}{\noalign{\hrule height 0.80pt}}

\newfont{\bb}{msbm10 scaled 1100}
\newcommand{\CC}{\mbox{\bb C}}
\newcommand{\PP}{\mbox{\bb P}}
\newcommand{\RR}{\mbox{\bb R}}
\newcommand{\QQ}{\mbox{\bb Q}}
\newcommand{\ZZ}{\mbox{\bb Z}}
\newcommand{\FF}{\mbox{\bb F}}
\newcommand{\GG}{\mbox{\bb G}}
\newcommand{\EE}{\mbox{\bb E}}
\newcommand{\NN}{\mbox{\bb N}}
\newcommand{\KK}{\mbox{\bb K}}

% Vectors

\newcommand{\av}{{\bf a}}
\newcommand{\bv}{{\bf b}}
\newcommand{\cv}{{\bf c}}
\newcommand{\dv}{{\bf d}}
\newcommand{\ev}{{\bf e}}
\newcommand{\fv}{{\bf f}}
\newcommand{\gv}{{\bf g}}
\newcommand{\hv}{{\bf h}}
\newcommand{\iv}{{\bf i}}
\newcommand{\jv}{{\bf j}}
\newcommand{\kv}{{\bf k}}
\newcommand{\lv}{{\bf l}}
\newcommand{\mv}{{\bf m}}
\newcommand{\nv}{{\bf n}}
\newcommand{\ov}{{\bf o}}
\newcommand{\pv}{{\bf p}}
\newcommand{\qv}{{\bf q}}
\newcommand{\rv}{{\bf r}}
\newcommand{\sv}{{\bf s}}
\newcommand{\tv}{{\bf t}}
\newcommand{\uv}{{\bf u}}
\newcommand{\wv}{{\bf w}}
\newcommand{\vv}{{\bf v}}
\newcommand{\xv}{{\bf x}}
\newcommand{\yv}{{\bf y}}
\newcommand{\zv}{{\bf z}}
\newcommand{\zerov}{{\bf 0}}
\newcommand{\onev}{{\bf 1}}

\def\u{{\bf u}}

% Matrices

\newcommand{\Am}{{\bf A}}
\newcommand{\Bm}{{\bf B}}
\newcommand{\Cm}{{\bf C}}
\newcommand{\Dm}{{\bf D}}
\newcommand{\Em}{{\bf E}}
\newcommand{\Fm}{{\bf F}}
\newcommand{\Gm}{{\bf G}}
\newcommand{\Hm}{{\bf H}}
\newcommand{\Id}{{\bf I}}
\newcommand{\Jm}{{\bf J}}
\newcommand{\Km}{{\bf K}}
\newcommand{\Lm}{{\bf L}}
\newcommand{\Mm}{{\bf M}}
\newcommand{\Nm}{{\bf N}}
\newcommand{\Om}{{\bf O}}
\newcommand{\Pm}{{\bf P}}
\newcommand{\Qm}{{\bf Q}}
\newcommand{\Rm}{{\bf R}}
\newcommand{\Sm}{{\bf S}}
\newcommand{\Tm}{{\bf T}}
\newcommand{\Um}{{\bf U}}
\newcommand{\Wm}{{\bf W}}
\newcommand{\Vm}{{\bf V}}
\newcommand{\Xm}{{\bf X}}
\newcommand{\Ym}{{\bf Y}}
\newcommand{\Zm}{{\bf Z}}
\newcommand{\Onem}{{\bf 1}}
\newcommand{\Zerom}{{\bf 0}}

% Calligraphic

\newcommand{\Acal}{{\cal A}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\Cc}{{\cal C}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Gc}{{\cal G}}
\newcommand{\Hc}{{\cal H}}
\newcommand{\Ic}{{\cal I}}
\newcommand{\Jc}{{\cal J}}
\newcommand{\Kc}{{\cal K}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Mc}{{\cal M}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Oc}{{\cal O}}
\newcommand{\Pc}{{\cal P}}
\newcommand{\Qc}{{\cal Q}}
\newcommand{\Rc}{{\cal R}}
\newcommand{\Sc}{{\cal S}}
\newcommand{\Tc}{{\cal T}}
\newcommand{\Uc}{{\cal U}}
\newcommand{\Wc}{{\cal W}}
\newcommand{\Vc}{{\cal V}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Zc}{{\cal Z}}

% Bold greek letters

\newcommand{\alphav}{\hbox{\boldmath$\alpha$}}
\newcommand{\betav}{\hbox{\boldmath$\beta$}}
\newcommand{\gammav}{\hbox{\boldmath$\gamma$}}
\newcommand{\deltav}{\hbox{\boldmath$\delta$}}
\newcommand{\etav}{\hbox{\boldmath$\eta$}}
\newcommand{\lambdav}{\hbox{\boldmath$\lambda$}}
\newcommand{\kappav}{\hbox{\boldmath$\kappa$}}
\newcommand{\epsilonv}{\hbox{\boldmath$\epsilon$}}
\newcommand{\nuv}{\hbox{\boldmath$\nu$}}
\newcommand{\muv}{\hbox{\boldmath$\mu$}}
\newcommand{\zetav}{\hbox{\boldmath$\zeta$}}
\newcommand{\phiv}{\hbox{\boldmath$\phi$}}
\newcommand{\psiv}{\hbox{\boldmath$\psi$}}
\newcommand{\thetav}{\hbox{\boldmath$\theta$}}
\newcommand{\tauv}{\hbox{\boldmath$\tau$}}
\newcommand{\omegav}{\hbox{\boldmath$\omega$}}
\newcommand{\xiv}{\hbox{\boldmath$\xi$}}
\newcommand{\sigmav}{\hbox{\boldmath$\sigma$}}
\newcommand{\piv}{\hbox{\boldmath$\pi$}}
\newcommand{\rhov}{\hbox{\boldmath$\rho$}}

\newcommand{\varthetav}{\hbox{\boldmath$\vartheta$}}
\newcommand{\varphiv}{\hbox{\boldmath$\varphi$}}
% \newcommand{\vtv}{\hbox{$\boldsymbol{\vartheta}$}}
% \newcommand{\vpv}{\hbox{$\boldsymbol{\varphi}$}}
\newcommand{\vpv}{\boldsymbol{\varphi}}
\newcommand{\vtv}{\boldsymbol{\vartheta}}


\newcommand{\Gammam}{\hbox{\boldmath$\Gamma$}}
\newcommand{\Lambdam}{\hbox{\boldmath$\Lambda$}}
\newcommand{\Deltam}{\hbox{\boldmath$\Delta$}}
\newcommand{\Sigmam}{\hbox{\boldmath$\Sigma$}}
\newcommand{\Phim}{\hbox{\boldmath$\Phi$}}
\newcommand{\Pim}{\hbox{\boldmath$\Pi$}}
\newcommand{\Psim}{\hbox{\boldmath$\Psi$}}
\newcommand{\psim}{\hbox{\boldmath$\psi$}}
\newcommand{\chim}{\hbox{\boldmath$\chi$}}
\newcommand{\omegam}{\hbox{\boldmath$\omega$}}
\newcommand{\Thetam}{\hbox{\boldmath$\Theta$}}
\newcommand{\Omegam}{\hbox{\boldmath$\Omega$}}
\newcommand{\Xim}{\hbox{\boldmath$\Xi$}}

% mixed symbols

\newcommand{\sinc}{{\hbox{sinc}}}
\newcommand{\diag}{{\hbox{diag}}}
\renewcommand{\det}{{\hbox{det}}}
\newcommand{\trace}{{\hbox{tr}}}
\newcommand{\sign}{{\hbox{sign}}}
\renewcommand{\arg}{{\hbox{arg}}}
\newcommand{\var}{{\hbox{var}}}
\newcommand{\cov}{{\hbox{cov}}}
\newcommand{\SINR}{{\sf sinr}}
\newcommand{\SNR}{{\sf snr}}
\newcommand{\Ei}{{\rm E}_{\rm i}}
%\renewcommand{\Re}{{\rm Re}}
%\renewcommand{\Im}{{\rm Im}}
\newcommand{\eqdef}{\stackrel{\Delta}{=}}
\newcommand{\defines}{{\,\,\stackrel{\scriptscriptstyle \bigtriangleup}{=}\,\,}}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}
\newcommand{\herm}{{\sf H}}
\newcommand{\trasp}{{\sf T}}
\renewcommand{\vec}{{\rm vec}}
\newcommand{\transp}{{\sf T}}
\newcommand{\calL}{\mbox{${\mathcal L}$}}
\newcommand{\calO}{\mbox{${\mathcal O}$}}


% \newcommand{\Ac}{\mbox{${\mathcal{A}}$}}
% \newcommand{\Hc}{\mbox{${\mathcal{A}}$}}

\newcommand{\Abc}{\mbox{$\boldsymbol{\mathcal{A}}$}}
\newcommand{\Bbc}{\mbox{$\boldsymbol{\mathcal{B}}$}}
\newcommand{\Cfd}{\mbox{$\boldsymbol{\mathcal{C}}$}}
\newcommand{\Dfd}{\mbox{$\boldsymbol{\mathcal{D}}$}}
\newcommand{\Efd}{\mbox{$\boldsymbol{\mathcal{E}}$}}
\newcommand{\Ffd}{\mbox{$\boldsymbol{\mathcal{F}}$}}
\newcommand{\Gfd}{\mbox{$\boldsymbol{\mathcal{G}}$}}
\newcommand{\Hbc}{\mbox{$\boldsymbol{\mathcal{H}}$}}
\newcommand{\Ifd}{\mbox{$\boldsymbol{\mathcal{I}}$}}
\newcommand{\Jfd}{\mbox{$\boldsymbol{\mathcal{J}}$}}
\newcommand{\Kfd}{\mbox{$\boldsymbol{\mathcal{K}}$}}
\newcommand{\Lfd}{\mbox{$\boldsymbol{\mathcal{L}}$}}
\newcommand{\Mfd}{\mbox{$\boldsymbol{\mathcal{M}}$}}
\newcommand{\Nfd}{\mbox{$\boldsymbol{\mathcal{N}}$}}
\newcommand{\Ofd}{\mbox{$\boldsymbol{\mathcal{O}}$}}
\newcommand{\Pfd}{\mbox{$\boldsymbol{\mathcal{P}}$}}
\newcommand{\Qfd}{\mbox{$\boldsymbol{\mathcal{Q}}$}}
\newcommand{\Rfd}{\mbox{$\boldsymbol{\mathcal{R}}$}}
\newcommand{\Sfd}{\mbox{$\boldsymbol{\mathcal{S}}$}}
\newcommand{\Tfd}{\mbox{$\boldsymbol{\mathcal{T}}$}}
\newcommand{\Ufd}{\mbox{$\boldsymbol{\mathcal{U}}$}}
\newcommand{\Vfd}{\mbox{$\boldsymbol{\mathcal{V}}$}}
\newcommand{\Wfd}{\mbox{$\boldsymbol{\mathcal{W}}$}}
\newcommand{\Xfd}{\mbox{$\boldsymbol{\mathcal{X}}$}}
\newcommand{\Yfd}{\mbox{$\boldsymbol{\mathcal{Y}}$}}
\newcommand{\Zfd}{\mbox{$\boldsymbol{\mathcal{Z}}$}}


